Learning to Rank Ace Neural Architectures via Normalized Discounted Cumulative Gain

One of the key challenges in Neural Architecture Search (NAS) is to efficiently rank the performances of architectures. The mainstream assessment of performance rankers uses ranking correlations (e.g., Kendall's tau), which pay equal attention to the whole space. However, the optimization goal of NAS is identifying top architectures while paying less attention on other architectures in the search space. In this paper, we show both empirically and theoretically that Normalized Discounted Cumulative Gain (NDCG) is a better metric for rankers. Subsequently, we propose a new algorithm, AceNAS, which directly optimizes NDCG with LambdaRank. It also leverages weak labels produced by weight-sharing NAS to pre-train the ranker, so as to further reduce search cost. Extensive experiments on 12 NAS benchmarks and a large-scale search space demonstrate that our approach consistently outperforms SOTA NAS methods, with up to 3.67% accuracy improvement and 8x reduction on search cost.

==> discussion.tex <==

\section{Discussion}

\subsection{Effectiveness of pretraining}

We further investigate in the capacity of our model, wondering how our GCN is good at capturing the information in the pretraning stage, WS-accuracy, FLOPs and parameters respectively. Apart from 4k architectures that are used in training, we sample extra 1k architectures per search space to evaluate the model. We compute $R^2$ scores to estimate the capability, as shown in \autoref{tab:pretrain-quality}. We found that for parameters and FLOPs, our GCN hits $>0.98$ for all search spaces, which means the model is very good at predicting the model size. However, on WS-accuracy, $R^2$ scores seem to be much lower. Although on NAS-Bench-101 and NAS-Bench-201, it still seems more than 0.9, on other  benchmarks it can be as low as 0.46. We hypothesis that architectures provided in NDS benchmark are more closer to each other, and the differences might be noisier. However, these are all at least good signs that GCN is actually learning information from weight-sharing labels.

\begin{table}
\centering
\begin{tabular}{cccc}
\toprule
        Search space & WS-accuracy & Parameters & FLOPs \\
\midrule
         NASNet &       0.576303 &         0.990884 &        0.990863 \\
          DARTS &       0.510170 &         0.994391 &        0.994508 \\
 NB201-CIFAR100 &       0.988104 &         0.999175 &        0.999158 \\
           PNAS &       0.619569 &         0.992423 &        0.992505 \\
           ENAS &       0.463366 &         0.984585 &        0.983611 \\
         Amoeba &       0.670243 &         0.993306 &        0.993134 \\
  NAS-Bench-101 &       0.937375 &         0.994931 &        0.994874 \\
  NB201-CIFAR10 &       0.988811 &         0.999287 &        0.999218 \\
   PNAS-fix-w-d &       0.624681 &         0.994920 &        0.994041 \\
 NB201-ImageNet &       0.981541 &         0.999121 &        0.999059 \\
   ENAS-fix-w-d &       0.649885 &         0.991492 &        0.993567 \\
  DARTS-fix-w-d &       0.450565 &         0.995128 &        0.995136 \\
\bottomrule
\end{tabular}
\caption{Performance ($R^2$-score) of GCN on predicting the WS-accuracy, parameters and FLOPs of architectures.}
\label{tab:pretrain-quality}
\end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/pretrain-quality.png}
%     \caption{Performance ($R^2$-score) of GCN on predicting the WS-accuracy, parameters and FLOPs of architectures.}
%     \label{fig:pretrain-quality}
% \end{figure}

From the perspective of weight-sharing, our method can be seen as one of those that leverage weight sharing as a start point. Rather than perform a greedy search guided by weight sharing~\cite{pourchot2020share} (\ie, to evaluate architectures in the order that is defined in weight-sharing), we iteratively select architectures to construct a ranking model and use the ranking model to further improve the selection. Therefore, we compare our methods against weight-sharing-guided greedy search. We set the budget to 100 architectures. For weight-sharing methods, as there is no ground truth needed, we directly pick the top-100 best performing architectures on super-net. For NASRank, we split the 100 budget into 80 and 20, where 80 models are sampled via iterative sampling and we report the best of the 20 models predicted finally. As shown in \autoref{fig:weight-sharing-comparison}, our method outcompetes weight-sharing greedy by a clear margin. especially on NAS-Bench-201, where our method is better on test regret by over 3\%. This echoes the result in \cite{zhang2020does} that weight-sharing has a steady bias towards the search space. We conjecture that such bias can be corrected with another model who has seen some architectures' real accuracy.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/weight-sharing-comparison.png}
    \caption{Comparison between weight-sharing-guided greedy search and NASRank with budget equals to 110. For weight-sharing greedy, 110 extra architectures are sampled and trained from scratch. For NASRank, 110 architectures are used to train the predictor, and 10 extra are selected at the final step. We report the test regret in the figure.}
    \label{fig:weight-sharing-comparison}
\end{figure}


% \begin{table}[htbp]
% \centering
% \begin{tabular}{ccc}
% \toprule
% Search space & Weight-sharing & NASRank \\
% \midrule
% NAS-Bench-101 & 0.47 & \meanstddiff{0.13}{0.47}{+0.34} \\
% NB201-CIFAR100 & 3.93 & \meanstddiff{0.17}{3.93}{+3.76} \\
% NB201-CIFAR10 & 0.79 & \meanstddiff{-0.10}{0.79}{+0.89} \\
% NB201-ImageNet & 0.75 & \meanstddiff{0.04}{0.75}{+0.71} \\
% Amoeba & 0.13 & \meanstddiff{0.08}{0.13}{+0.05} \\
% DARTS & 0.18 & \meanstddiff{0.18}{0.18}{+0.00} \\
% DARTS-fix-w-d & 0.29 & \meanstddiff{0.14}{0.29}{+0.14} \\
% ENAS & 0.38 & \meanstddiff{0.27}{0.38}{+0.11} \\
% ENAS-fix-w-d & 0.14 & \meanstddiff{0.03}{0.14}{+0.11} \\
% NASNet & 0.36 & \meanstddiff{0.32}{0.36}{+0.04} \\
% PNAS & 0.34 & \meanstddiff{0.13}{0.34}{+0.21} \\
% PNAS-fix-w-d & 0.11 & \meanstddiff{0.15}{0.11}{-0.04} \\
% \bottomrule
% \end{tabular}
% \caption{Comparison between pure weight sharing and NASRank with budget equals to 110. For weight sharing, 110 extra architectures are sampled and trained from scratch. For NASRank, 110 architectures are used to train the predictor, and 10 extra are selected at the final step. We report the test regret in the table.}
% \label{tab:weight-sharing-comparison}
% \end{table}

% \lz{why select weight-sharing as comparison baseline?In abstract and section3: we use and leverage weight sharing}

% \lz{If NASRank is a performance predictor, we should compare with different performance predictors}


\subsection{Effectiveness of NDCG}

